Learning nonlinear feedforward: a Gaussian Process Approach Applied to a Printer with Friction

Feedforward control is essential to achieving good tracking performance in positioning systems. The aim of this paper is to develop an identification strategy for inverse models of systems with nonlinear dynamics of unknown structure using input-output data, which directly delivers feedforward signals for a-priori unknown tasks. To this end, inverse systems are regarded as noncausal nonlinear finite impulse response (NFIR) systems and modeled as a Gaussian Process with a stationary kernel function that imposes properties such as smoothness and periodicity. The approach is validated experimentally on a consumer printer with friction and shown to lead to improved tracking performance with respect to linear feedforward.

==> ACC submission Arxiv/tikz_set.tex <==
% In mail tex file:
% 		\input{tikz_set}

% Use in caption as:
% (\protect\bluedot)


\usepackage{tikz}
\usepackage{tikzscale}

%max: 
% % \usepackage{pgfplots} 
% % \pgfplotsset{compat=newest} 
% % \pgfplotsset{plot coordinates/math parser=false} 
% % \newlength\figureheight 
% % \newlength\figurewidth 
% % \newlength\defcolwidth

% \setlength\defcolwidth{7.85cm}
% \setlength\figurewidth{.6\defcolwidth}
% \setlength\figureheight{.7\figurewidth}
%%
\definecolor{myorange}{cmyk}{0,0.35,0.85,0} 
\definecolor{mypurple}{cmyk}{0.5,1,0,0} 

\definecolor{matblue1}{rgb}{0,0.4470,0.7410}
\definecolor{matred1}{rgb}{0.85,0.325,0.098}
\definecolor{matyel1}{rgb}{0.9290, 0.6940, 0.1250}
\definecolor{matpur1}{rgb}{0.4940, 0.1840, 0.5560}
\definecolor{matgre1}{rgb}{0.4660, 0.6740, 0.1880}
\definecolor{matblue2}{rgb}{0.3010, 0.7450, 0.9330}
\definecolor{matred2}{rgb}{0.6350, 0.0780, 0.1840}
\definecolor{matgrey1}{rgb}{0.5, 0.6, 0.7}
\definecolor{matpink1}{rgb}{1, 0.07, 0.65}
\definecolor{matblue3}{rgb}{0.07, 0.62, 1}
\definecolor{gray09}{rgb}{0.9, 0.9, 0.9}

% added by Noud
    \definecolor{mblue}{rgb}{0,0.447,0.741}
    \definecolor{mred}{rgb}{0.85,0.325,0.098}
    \definecolor{myellow}{rgb}{0.9290,0.6940,0.1250}
    \definecolor{mmagenta}{rgb}{1,0,1}
    \definecolor{mgreen}{rgb}{0.4460,0.6740,0.1880}
    \definecolor{mgrey}{rgb}{0.6,0.6,0.6}
    \definecolor{mpurple}{rgb}{0.4940, 0.1840, 0.5560}
    
    \tikzset{cross/.style={cross out, draw=black, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt}, cross/.default={1pt}}
    
    \usetikzlibrary{shapes}
	
%

\newcommand{\bluedashdot}{\raisebox{2pt}{\tikz{\draw[-,matblue1,densely dash dot,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\blackdashdot}{\raisebox{2pt}{\tikz{\draw[-,black,densely dash dot,line width = 0.9pt](0,0) -- (3mm,0);}}}

\newcommand{\bluedots}{\raisebox{2pt}{\tikz{\draw[-,matblue1,densely dotted,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\blackdots}{\raisebox{2pt}{\tikz{\draw[-,black,densely dotted,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\yeldots}{\raisebox{2pt}{\tikz{\draw[-,matyel1,densely dotted,line width = 0.9pt](0,0) -- (3mm,0);}}}

\newcommand{\reddash}{\raisebox{2pt}{\tikz{\draw[-,matred1,dashed,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\yeldash}{\raisebox{2pt}{\tikz{\draw[-,matyel1,dashed,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\bluedash}{\raisebox{2pt}{\tikz{\draw[-,matblue1,dashed,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\greendash}{\raisebox{2pt}{\tikz{\draw[-,ForestGreen,dashed,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\blackdash}{\raisebox{2pt}{\tikz{\draw[-,black,dashed,line width = 0.9pt](0,0) -- (3mm,0);}}}

\newcommand{\blackline}{\raisebox{2pt}{\tikz{\draw[-,black,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\blueline}{\raisebox{2pt}{\tikz{\draw[-,matblue1,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\redline}{\raisebox{2pt}{\tikz{\draw[-,matred1,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\orangeline}{\raisebox{2pt}{\tikz{\draw[-,myorange,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\purpleline}{\raisebox{2pt}{\tikz{\draw[-,mypurple,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}

\newcommand{\bluedot}{\raisebox{.7pt}{\tikz{\draw[-,matblue1,solid,line width = 1pt](0,0) circle (.7mm);}}}
\newcommand{\reddot}{\raisebox{.7pt}{\tikz{\draw[-,matred1,solid,line width = 1pt](0,0) circle (.7mm);}}}
\newcommand{\yeldot}{\raisebox{.7pt}{\tikz{\draw[-,matyel1,solid,line width = 1pt](0,0) circle (.7mm);}}}
\newcommand{\purdot}{\raisebox{.7pt}{\tikz{\draw[-,matpur1,solid,line width = 1pt](0,0) circle (.7mm);}}}
\newcommand{\gredot}{\raisebox{.7pt}{\tikz{\draw[-,matgre1,solid,line width = 1pt](0,0) circle (.7mm);}}}
\newcommand{\bluedott}{\raisebox{.7pt}{\tikz{\draw[-,matblue2,solid,line width = 1pt](0,0) circle (.7mm);}}}
\newcommand{\reddott}{\raisebox{.7pt}{\tikz{\draw[-,matred2,solid,line width = 1pt](0,0) circle (.7mm);}}}
\newcommand{\greydot}{\raisebox{.7pt}{\tikz{\draw[-,matgrey1,solid,line width = 1pt](0,0) circle (.7mm);}}}
\newcommand{\pinkdot}{\raisebox{.7pt}{\tikz{\draw[-,matpink1,solid,line width = 1pt](0,0) circle (.7mm);}}}
\newcommand{\bluedottt}{\raisebox{.7pt}{\tikz{\draw[-,matblue3,solid,line width = 1pt](0,0) circle (.7mm);}}}

\newcommand{\yelline}{\raisebox{2pt}{\tikz{\draw[-,matyel1,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\purline}{\raisebox{2pt}{\tikz{\draw[-,matpur1,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\greenline}{\raisebox{2pt}{\tikz{\draw[-,matgre1,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\bluelinet}{\raisebox{2pt}{\tikz{\draw[-,matblue2,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}
\newcommand{\redlinet}{\raisebox{2pt}{\tikz{\draw[-,matred2,solid,line width = 0.9pt](0,0) -- (3mm,0);}}}


\newcommand{\greyarea}{\raisebox{0pt}{\tikz{\draw[-,gray09,solid,line width = 4pt](0,0) -- (3mm,0);}}}

%\tikzset{cross/.style={cross out, draw=black, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt}, cross/.default={0.9pt}}

\newcommand{\blackcross}{
\tikz{
	\filldraw (0,0) node[cross] {};
}}
\newcommand{\redtriangle}{
\tikz{
    \filldraw[-,matred1,solid,line width=0.9pt](-0.12,0) -- (0,0.24) -- (0.12,0) -- (-0.12,0) -- cycle;
}}

\newcommand{\bluetriangle}{
\begin{tikzpicture}
    \draw[-,matblue1,solid,line width=0.9pt](0,0) -- (0.12,0.24) -- (0.24,0) -- (0,0) -- cycle;
    \draw[-,matblue1,dashed,line width = 0.9pt](-0.2,0.1) -- (0.44,0.1);
\end{tikzpicture}}


\newcommand{\yelcircle}{\begin{tikzpicture}
    \draw[-,matyel1,solid,line width=0.9pt] (0.12,0.12) circle [radius=0.12];
    \draw[-,matyel1,dashed,line width = 0.9pt](-0.2,0.12) -- (0.44,0.12);
\end{tikzpicture}}

\newcommand{\redcircle}{\begin{tikzpicture}
    \draw[-,matred1,solid,line width=0.9pt] (0.12,0.12) circle [radius=0.12];
    \draw[-,matred1,dashed,line width = 0.9pt](-0.2,0.12) -- (0.44,0.12);
\end{tikzpicture}}


